F-FDN: Federation of Fog Computing Systems for Low Latency Video Streaming

Video streaming is growing in popularity and has become the most bandwidth-consuming Internet service. As such, robust streaming in terms of low latency and uninterrupted streaming experience, particularly for viewers in distant areas, has become a challenge. The common practice to reduce latency is to pre-process multiple versions of each video and use Content Delivery Networks (CDN) to cache videos that are popular in a geographical area. However, with the fast-growing video repository sizes, caching video contents in multiple versions on each CDN is becoming inefficient. Accordingly, in this paper, we propose the architecture for Fog Delivery Networks (FDN) and provide methods to federate them (called F-FDN) to reduce video streaming latency. In addition to caching, FDNs have the ability to process videos in an on-demand manner. F-FDN leverages cached contents on the neighboring FDNs to further reduce latency. In particular, F-FDN is equipped with methods that aim at reducing latency through probabilistically evaluating the cost benefit of fetching video segments either from neighboring FDNs or by processing them. Experimental results against alternative streaming methods show that both on-demand processing and leveraging cached video segments on neighboring FDNs can remarkably reduce streaming latency (on average 52%).

==> Sources/sec-apndx.tex <==
\section{Appendix}\label{sec:apndx}

\begin{lemma}
\label{LeftCosetsDisjoint}
Let $N$, $C(k)$, and $S(k)$ be the total number of network nodes, compromised set of nodes, and secure (non-compromised) network nodes, respectively. Also, we define $V$ and $\beta(k)$ to be, respectively, the vulnerability factor, and the number of network nodes which get compromised at the $k$-th step during the MDP generation phase. 
Then
\begin{equation}
\beta(k+1) = N\cdot\big(\frac{N-V}{N}\big)^{\frac{\log(1-\frac{C(k)}{N})}{\log(\frac{N-V}{N})}}\cdot\Big[ 1 - \big(\frac{N-V}{N}\big)^{\beta(k)} \Big],
\end{equation}

\end{lemma}

\begin{IEEEproof}
Clearly, the number of internal compromised network nodes is initially zero, i.e., $C(0) = 0$. Given the vulnerability factor of $V$, the next step of the MDP generation will result in $C(1) = V$, i.e., $V$ new MDP states. Next, \name will use each of the $V$ compromised nodes, and the non-compromised hosts which are accessible from any of those $V$ compromised nodes, to further expand the MDP model. It is important to mention that exploration of every compromised node will result in $\leq V$ new compromised nodes as some them may have already been compromised during one of the previous steps. 

We calculate the expected number of non-compromised network nodes which are visited (get compromised) at the $k$-th step of the MDP generation procedure, i.e., $\beta(k+1)$. Clearly, those network nodes are visited through investigation of the nodes which got newly compromised during the previous phase $\beta(k)$. Once the first node out of the $\beta(k)$ nodes is investigated, the expected number of compromised nodes is $E[c_k(1)] = C(k) + V\cdot\frac{N-C(k)}{N}$, where $V\cdot\frac{N-V}{N}$ new nodes are compromised, because $V$ (vulnerability factor) nodes are selected which are each non-compromised with probability $\frac{N-V}{N}$. Following some algebraic calculations and arrangements, we have the closed form solution 
\begin{equation}
c_0(n) = N\cdot\Big[1-\big(\frac{N-V}{N}\big)^{n}\Big],
\end{equation}
and hence, we calculate $\beta(k+1)$ as $C(k+1) - C(k)$:
\begin{equation}
\beta(k+1) = N\cdot\big(\frac{N-V}{N}\big)^\alpha\cdot\Big[ 1 - \big(\frac{N-V}{N}\big)^{\beta(k)} \Big],
\end{equation}
where
\begin{equation}
\alpha = \frac{\log(1-\frac{C(k)}{N})}{\log(\frac{N-V}{N})}.
\end{equation}

\qed
\end{IEEEproof}
